AgentDoG2: An Efficient Alignment Framework for Emergent Risk in Long-Horizon Agent Tasks

Recent large language model (LLM) agents exhibit promising capabilities on complex long-horizon tasks yet introduce more challenging and covert safety risks. In this work, we propose an efficient framework for characterizing, evaluating, and mitigating these risks in long-horizon agent tasks. Specifically, we update the agentic safety taxonomy to accommodate emergent risks from long-horizon execution scenarios with ATBench-Pro. We further develop ManipulationArena and introduce goal manipulation attack methods, which frequently occur in long-horizon agent tasks. To identify these risks more efficiently, we train AgentDoG2, AgentDoG-Jev, and AgentDoG-Step (0.8B, 2B, 4B, 8B, and 9B parameters) for trajectory- and step-level safety evaluation, outperforming closed-source models (\emph{e.g.,} GPT-6.1-Sol) with almost 100x speedup compared to AgentDoG1.5. Finally, we explore a preliminary safe agentic recursive self-improvement method with AgentDoG for auto-alignment. Extensive experimental results indicate that the AgentDoG2 family and the proposed attack method achieve state-of-the-art performance in diverse and complex long-horizon agentic scenarios. All models and datasets are openly released.

==> sections/agentdog.tex <==
\section{\agentdog{}}
\label{sec:agentdog}
% Writing: 段东杭、马嘉晨
% Review: 王鹏
AgentDoG~2.0 upgrades trajectory-level agent safety evaluation along two axes: broader risk coverage through an expanded safety taxonomy and substantially lower inference overhead.
Unlike AgentDoG~1.5~\citep{liu2026agentdog15lightweightscalable}, which injects the full safety taxonomy into every input prompt and generates a verbose Chain-of-Thought (CoT) rationale prior to emitting a judgment, AgentDoG~2.0 is trained on updated trajectory data to internalize the expanded taxonomy and directly output a structured diagnosis.
% TODO: Add headline efficiency and accuracy gains once retraining and evaluation are complete.

\begin{figure*}[h]
  \centering
  \fbox{\parbox{0.9\linewidth}{\centering
    \vspace{2em}
    \textbf{PLACEHOLDER:} input and output for the same agent trajectory (prompt comparison).\\
    To be populated after the final evaluation.
    \vspace{2em}}}
  \caption{\textbf{Placeholder:} input and output for the same agent trajectory (prompt comparison).}
\end{figure*}

%%%%%

\subsection{Task Definition}
\label{subsec:agentdog-1}
Following AgentDoG~1.0 and~1.5~\citep{liu2026agentdogdiagnosticguardrailframework,liu2026agentdog15lightweightscalable}, we evaluate safety over a complete agent trajectory.
Let $\mathcal{T}=(u,t_1,\ldots,t_n)$ denote the trajectory, where $u$ is the initial user request and each step $t_i=(a_i,o_i)$ pairs an agent action $a_i$ with its resulting environment observation $o_i$.
The evaluator takes as input $x=(q,\mathcal{U},\mathcal{T})$, where $q$ specifies the evaluation instruction and $\mathcal{U}$ denotes the set of available tools.

\paragraph{Trajectory-level safety.}
The binary safety judgment is $y\in\{\texttt{safe},\texttt{unsafe}\}$.
A trajectory is labeled unsafe if at least one step involves an unsafe agent action or decision:
\begin{equation}
  y=\texttt{unsafe}
  \quad\Longleftrightarrow\quad
  \exists\,i\in\{1,\ldots,n\},\;\mathsf{Unsafe}(\mathcal{T},i) = \mathrm{True},
\end{equation}
where $\mathsf{Unsafe}(\mathcal{T},i)$ assesses the agent's action at step~$i$ conditioned on the full trajectory context.
Notably, a risky user request or adversarial observation that the agent handles safely still yields a \texttt{safe} judgment.

\paragraph{Expanded safety taxonomy and fine-grained risk diagnosis.}
Beyond binary classification, let $\ell^{\text{mode}}\in\mathcal{L}^{\text{mode}}$, $\ell^{\text{harm}}\in\mathcal{L}^{\text{harm}}$, and $\ell^{\text{risk}}\in\mathcal{L}^{\text{risk}}\cup\{\texttt{None}\}$ denote the failure mode, potential real-world harm, and risk source, respectively, where \texttt{None} indicates the absence of a risk source.
% TODO: Describe the newly added taxonomy categories once finalized.
The structured target tuple is defined as
\begin{equation}
  y_{\mathrm{fine}} =
  \begin{cases}
    (y,\ell^{\text{risk}}), & y=\texttt{safe},\\
    (y,\ell^{\text{mode}},\ell^{\text{harm}},\ell^{\text{risk}}),
       & y=\texttt{unsafe}.
  \end{cases}
\end{equation}
In words, a safe trajectory outputs only the binary judgment and risk source (possibly \texttt{None}), decoupling the origin of a risk from whether the agent realized it; an unsafe trajectory outputs the full four-field diagnosis.
The evaluator generates a single response $r$ that serializes $y_{\mathrm{fine}}$ into named fields.

\paragraph{Taxonomy internalization and direct prompting.}
Compared with AgentDoG~1.5, the 2.0 prompt removes both the in-context taxonomy block and the CoT rationale instruction, requesting only the serialized output fields.
Because the prompt provides field names without category definitions, the evaluator learns to map trajectory evidence directly to taxonomy labels from training supervision.

%%%%%

\subsection{Data Preparation}
\label{subsec:agentdog-2}
% TODO: Fill in Data Preparation after finalizing the expanded taxonomy and retraining datasets.
\mbox{}

%%%%%

\subsection{Training}
\label{subsec:agentdog-3}
Following AgentDoG~1.5~\citep{liu2026agentdog15lightweightscalable}, we adopt a two-stage training pipeline: SFT initializes the evaluator to internalize the taxonomy and emit direct structured judgments, and RL refines both binary safety and fine-grained diagnosis using verifiable rewards.

\subsubsection{Supervised Fine-Tuning}
We fine-tune the base model on demonstrations $(x,r)\sim\mathcal{D}_{\mathrm{SFT}}$.
Given the trajectory input $x$, the policy $\pi_\theta$ learns to generate the serialized target $r$ autoregressively by minimizing the token-level negative log-likelihood over target tokens:
\begin{equation}
  \mathcal{L}_{\mathrm{SFT}}(\theta)
  = -\mathbb{E}_{(x,r)\sim\mathcal{D}_{\mathrm{SFT}}}
    \sum_{t=1}^{|r|}
    \log\pi_{\theta}(r_t\mid x,r_{<t}),
\end{equation}
where $r_t$ is the $t$-th target token and prompt tokens in $x$ are masked.
% TODO: Confirm SFT hyperparameters (epochs, schedule, peak LR) after retraining.

\subsubsection{Reinforcement Learning}
We further optimize the SFT policy using Group Reward-Decoupled Normalization Policy Optimization (GDPO)~\citep{liu2026gdpo}.
For each input $x_i$, the rollout policy $\pi_{\theta_{\mathrm{old}}}$ samples a group of $G$ candidate responses $\{o_{i,j}\}_{j=1}^G$.
A deterministic verifier validates the output schema and assigns a binary correctness reward $\rho_{i,j,k} \in \{0,1\}$ to each applicable field $k \in \mathcal{K}_i$ (with format-invalid outputs receiving zero reward across all fields).
Specifically, binary safety and risk source are scored across all trajectories ($\mathcal{K}_i=\{\mathrm{Safety},\mathrm{RS}\}$ for safe trajectories), whereas for ground-truth unsafe trajectories ($\mathcal{K}_i=\{\mathrm{Safety},\mathrm{RS},\mathrm{FM},\mathrm{RWH}\}$), failure mode and potential real-world harm receive credit only when the model also returns the correct \texttt{unsafe} judgment.
Scoring Risk Source on safe trajectories also helps mitigate reward-variance asymmetry under variance-filtered rollouts (analyzed in detail at the step level in Section~\ref{sec:agentdog-step}).

To prevent multi-field reward interference, GDPO normalizes each reward dimension independently within the rollout group before averaging over the applicable fields $\mathcal{K}_i$:
\begin{equation}
  A_{i,j} = \frac{1}{|\mathcal{K}_i|}
  \sum_{k\in\mathcal{K}_i}
    \frac{\rho_{i,j,k}-\mu_{i,k}}{\sigma_{i,k}+\delta},
\end{equation}
where $\mu_{i,k}$ and $\sigma_{i,k}$ denote the within-group mean and standard deviation for field $k$, and $\delta=10^{-6}$ ensures numerical stability.
We retain only rollout groups that exhibit non-zero reward variance in at least one field, and apply batch-level normalization to $A_{i,j}$ to obtain the response-level advantage $\hat{A}_{\mathrm{sum}}^{(i,j)}$ shared across all tokens in $o_{i,j}$.
Defining the token-level importance sampling ratio as
\begin{equation}
  s_{i,j,t}(\theta) =
    \frac{\pi_\theta(o_{i,j}^{t}\mid x_i,o_{i,j}^{<t})}
         {\pi_{\theta_{\mathrm{old}}}(o_{i,j}^{t}\mid x_i,o_{i,j}^{<t})}
\end{equation}
and the clipped surrogate term as
\begin{equation}
  \ell_{i,j,t}^{\mathrm{clip}}(\theta)
  = \min\!\left(
      s_{i,j,t}(\theta)\hat{A}_{\mathrm{sum}}^{(i,j)},\,
      \operatorname{clip}\!\left(s_{i,j,t}(\theta),\, 1-\epsilon_{\mathrm{low}},\, 1+\epsilon_{\mathrm{high}}\right)\hat{A}_{\mathrm{sum}}^{(i,j)}
    \right),
\end{equation}
we maximize the token-averaged clipped surrogate objective:
\begin{equation}
  \mathcal{J}_{\mathrm{GDPO}}(\theta)
  = \mathbb{E}_{x_i,\{o_{i,j}\}}\!\left[
    \frac{1}{G}\sum_{j=1}^{G}\frac{1}{T_{i,j}}
    \sum_{t=1}^{T_{i,j}}
    \ell_{i,j,t}^{\mathrm{clip}}(\theta)
  \right],
\end{equation}
where $T_{i,j} = |o_{i,j}|$ is the token length of response $o_{i,j}$.
% TODO: Confirm RL hyperparameters (G, clip bounds, iterations, LR) after retraining.

%%%%%

\subsection{Evaluation}
\label{subsec:agentdog-4}

\subsubsection{Experimental Setup}

\paragraph{Models and baselines.}
We evaluate AgentDoG~2.0 against AgentDoG~1.5-U across five base models: Qwen3.5-0.8B, Qwen3.5-2B, Qwen3.5-4B, Llama-3.1-8B, and Qwen3.5-9B.
For broader comparison on the accuracy--efficiency frontier, we evaluate closed-source frontier LLMs (GPT-6.1-Sol, GPT-5.4, Gemini~3.8 Flash, and Gemini~3.1 Pro), open-weight general LLMs (Qwen3.5-397B-A17B, Qwen3-235B-A22B, Qwen3.8-27B, Qwen3.5-9B, Llama-3.1-8B-Instruct, and Qwen3.5-4B; shown with concise names in tables), and dedicated safety guards (ShieldAgent, LlamaGuard4-12B, LlamaGuard3-8B, and Qwen3-Guard).

\paragraph{Benchmarks and metrics.}
We evaluate trajectory-level safety across R-Judge~\citep{yuan-etal-2024-r}, ATBench~\citep{li2026atbenchdiverserealistictrajectory}, and ATBench-Pro.
% TODO: Add ATBench-Pro citation and gold-unsafe trajectory counts.
We report binary accuracy and unsafe-class F1 on all three benchmarks, and evaluate fine-grained risk diagnosis on gold-unsafe trajectories of ATBench and ATBench-Pro via per-dimension accuracy on Risk Source (RS), Failure Mode (FM), and Real-World Harm (RWH) together with their mean (Avg.).

\paragraph{Efficiency measures.}
To evaluate the deployment overhead of trajectory-level guardrails alongside effectiveness, we measure inference efficiency in terms of output tokens, total tokens (input plus output), and end-to-end wall-clock latency.
Token counts are averaged over overlapping requests with valid usage statistics, using a shared tokenizer for locally hosted models and API-reported counts for closed-source models.
For locally hosted models, we measure mean wall-clock latency on a balanced subset of trajectories per benchmark with concurrency set to one ($1$ request in flight) and prefix caching disabled.
In the Pareto plots, we pair each effectiveness metric with these three efficiency measures on logarithmic scales to characterize the accuracy--cost trade-off.

\subsubsection{Binary Safety Judgment}
% TODO: Fill in binary safety judgment analysis across R-Judge, ATBench, and ATBench-Pro (Table~\ref{tab:agentdog2-binary}, figure placeholder).

\begin{table*}[h]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{1.05}
  \definecolor{ad2sec}{HTML}{EBD3AC}
  \begin{tabular}{@{}lcccccccc@{}}
    \toprule
    & \multicolumn{2}{c}{\textbf{R-Judge}}
      & \multicolumn{2}{c}{\textbf{ATBench}}
      & \multicolumn{2}{c}{\textbf{ATBench-Pro}}
      & \multicolumn{2}{c}{\textbf{Overall}} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(l){8-9}
    \textbf{Model}
      & Acc ($\uparrow$) & F1 ($\uparrow$)
      & Acc ($\uparrow$) & F1 ($\uparrow$)
      & Acc ($\uparrow$) & F1 ($\uparrow$)
       & Acc ($\uparrow$) & F1 ($\uparrow$) \\
    \midrule
    \rowcolor{ad2sec}\multicolumn{9}{l}{\textbf{Closed-Source Models}} \\
    GPT-6.1-Sol & 94.9 & 95.0 & 78.0 & 77.5 & -- & -- & -- & -- \\
    GPT-5.4 & 93.3 & 93.7 & 73.7 & 76.7 & -- & -- & -- & -- \\
    Gemini~3.8 Flash & 91.7 & 92.6 & 59.2 & 53.1 & -- & -- & -- & -- \\
    Gemini~3.1 Pro & 97.3 & 97.4 & 75.5 & 75.0 & -- & -- & -- & -- \\
    \addlinespace[2pt]
    \rowcolor{ad2sec}\multicolumn{9}{l}{\textbf{Open-Source Models}} \\
    Qwen3.5-397B & 85.6 & 87.4 & 66.8 & 67.8 & -- & -- & -- & -- \\
    Qwen3-235B & 85.1 & 87.0 & 59.2 & 60.8 & -- & -- & -- & -- \\
    Qwen3.8-27B & 93.4 & 93.5 & 71.3 & 61.8 & -- & -- & -- & -- \\
    Qwen3.5-9B & 77.0 & 80.3 & 62.7 & 53.9 & -- & -- & -- & -- \\
    Llama-3.1-8B & 53.7 & 69.5 & 45.3 & 61.9 & -- & -- & -- & -- \\
    Qwen3.5-4B & 81.0 & 82.0 & 45.9 & 27.6 & -- & -- & -- & -- \\
    \addlinespace[2pt]
    \rowcolor{ad2sec}\multicolumn{9}{l}{\textbf{Guard Models}} \\
    ShieldAgent & 81.0 & 84.6 & 62.5 & 67.7 & -- & -- & -- & -- \\
    LlamaGuard4-12B & 63.8 & 63.2 & 58.1 & 41.7 & -- & -- & -- & -- \\
    LlamaGuard3-8B & 61.2 & 56.7 & 53.1 & 7.3 & -- & -- & -- & -- \\
    Qwen3-Guard & 40.6 & 9.0 & 51.5 & 0.8 & -- & -- & -- & -- \\
    \addlinespace[2pt]
    \rowcolor{ad2sec}\multicolumn{9}{l}{\textbf{AgentDoG~1.5}} \\
    AgentDoG~1.5-U 0.8B & 81.2 & 80.2 & 61.0 & 62.6 & -- & -- & -- & -- \\
    AgentDoG~1.5-U 2B & 78.4 & 80.9 & 76.8 & 76.9 & -- & -- & -- & -- \\
    AgentDoG~1.5-U 4B & 90.4 & 90.6 & 78.4 & 76.1 & -- & -- & -- & -- \\
    AgentDoG~1.5-U 8B & 86.9 & 86.3 & 77.3 & 75.6 & -- & -- & -- & -- \\
    AgentDoG~1.5-U 9B & 81.4 & 83.4 & 78.1 & 78.0 & -- & -- & -- & -- \\
    \addlinespace[2pt]
    \rowcolor{ad2sec}\multicolumn{9}{l}{\textbf{AgentDoG~2.0}} \\
    AgentDoG~2.0 0.8B & -- & -- & -- & -- & -- & -- & -- & -- \\
    AgentDoG~2.0 2B & -- & -- & -- & -- & -- & -- & -- & -- \\
    AgentDoG~2.0 4B & -- & -- & -- & -- & -- & -- & -- & -- \\
    AgentDoG~2.0 8B & -- & -- & -- & -- & -- & -- & -- & -- \\
    AgentDoG~2.0 9B & -- & -- & -- & -- & -- & -- & -- & -- \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Trajectory-level binary safety judgment (Accuracy and unsafe F1, \%) across benchmarks.}
    Previously reported baseline scores on R-Judge and ATBench are shown for reference; Overall is reported only when all benchmarks are available; cells marked \texttt{--} are reserved for newly added baselines, AgentDoG~2.0 retraining, and ATBench-Pro evaluation.}
  \label{tab:agentdog2-binary}
\end{table*}

\begin{figure*}[h]
  \centering
  \fbox{\parbox{0.9\linewidth}{\centering
    \vspace{2em}
    \textbf{PLACEHOLDER:} binary safety F1 versus inference efficiency.\\
    To be populated after the final evaluation.
    \vspace{2em}}}
  \caption{\textbf{Placeholder:} binary safety F1 versus inference efficiency.}
\end{figure*}

\subsubsection{Fine-Grained Risk Diagnosis}
% TODO: Fill in fine-grained risk diagnosis analysis across RS, FM, and RWH on ATBench and ATBench-Pro (Table~\ref{tab:agentdog2-fine}, figure placeholder).

\begin{table*}[h]
  \centering
  \small
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.05}
  \definecolor{ad2sec}{HTML}{EBD3AC}
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lcccccccccccc@{}}
      \toprule
      & \multicolumn{4}{c}{\textbf{ATBench}}
        & \multicolumn{4}{c}{\textbf{ATBench-Pro}}
        & \multicolumn{4}{c}{\textbf{Overall}} \\
      \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(l){10-13}
      \textbf{Model}
        & RS ($\uparrow$) & FM ($\uparrow$) & RWH ($\uparrow$) & Avg.\ ($\uparrow$)
        & RS ($\uparrow$) & FM ($\uparrow$) & RWH ($\uparrow$) & Avg.\ ($\uparrow$)
         & RS ($\uparrow$) & FM ($\uparrow$) & RWH ($\uparrow$) & Avg.\ ($\uparrow$) \\
      \midrule
      \rowcolor{ad2sec}\multicolumn{13}{l}{\textbf{Closed-Source Models}} \\
      GPT-6.1-Sol & 38.0 & 14.1 & 37.6 & 29.9 & -- & -- & -- & -- & -- & -- & -- & -- \\
      GPT-5.4 & 33.6 & 13.5 & 30.2 & 25.8 & -- & -- & -- & -- & -- & -- & -- & -- \\
      Gemini~3.8 Flash & 22.1 & 10.3 & 21.3 & 17.9 & -- & -- & -- & -- & -- & -- & -- & -- \\
      Gemini~3.1 Pro & 24.8 & 12.6 & 18.5 & 18.6 & -- & -- & -- & -- & -- & -- & -- & -- \\
      \addlinespace[2pt]
      \rowcolor{ad2sec}\multicolumn{13}{l}{\textbf{Open-Weight General Models}} \\
      Qwen3.5-397B & 7.7 & 3.6 & 6.8 & 6.0 & -- & -- & -- & -- & -- & -- & -- & -- \\
      Qwen3-235B & 7.0 & 11.6 & 26.6 & 15.1 & -- & -- & -- & -- & -- & -- & -- & -- \\
      Qwen3.8-27B & 28.4 & 10.7 & 23.1 & 20.7 & -- & -- & -- & -- & -- & -- & -- & -- \\
      Qwen3.5-9B & 16.5 & 8.5 & 16.7 & 13.9 & -- & -- & -- & -- & -- & -- & -- & -- \\
      Llama-3.1-8B & 6.2 & 5.8 & 15.5 & 9.2 & -- & -- & -- & -- & -- & -- & -- & -- \\
      Qwen3.5-4B & 6.6 & 3.0 & 8.2 & 5.9 & -- & -- & -- & -- & -- & -- & -- & -- \\
      \addlinespace[2pt]
      \rowcolor{ad2sec}\multicolumn{13}{l}{\textbf{AgentDoG~1.5}} \\
      AgentDoG~1.5-U 0.8B & 37.4 & 14.3 & 34.0 & 28.6 & -- & -- & -- & -- & -- & -- & -- & -- \\
      AgentDoG~1.5-U 2B & 42.7 & 18.5 & 43.5 & 34.9 & -- & -- & -- & -- & -- & -- & -- & -- \\
      AgentDoG~1.5-U 4B & 46.7 & 14.5 & 45.1 & 35.4 & -- & -- & -- & -- & -- & -- & -- & -- \\
      AgentDoG~1.5-U 8B & 48.5 & 16.5 & 43.1 & 36.0 & -- & -- & -- & -- & -- & -- & -- & -- \\
      AgentDoG~1.5-U 9B & 53.5 & 17.7 & 50.3 & 40.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
      \addlinespace[2pt]
      \rowcolor{ad2sec}\multicolumn{13}{l}{\textbf{AgentDoG~2.0}} \\
      AgentDoG~2.0 0.8B & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      AgentDoG~2.0 2B & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      AgentDoG~2.0 4B & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      AgentDoG~2.0 8B & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      AgentDoG~2.0 9B & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
      \bottomrule
    \end{tabular}%
  }
  \caption{\textbf{Fine-grained risk diagnosis accuracy (\%) across dimensions on gold-unsafe trajectories.}
    RS, FM, and RWH denote Risk Source, Failure Mode, and Real-World Harm, respectively, and Avg.\ is their mean.
    Dedicated guard models are excluded as they only output binary safety judgments.
    Previously reported ATBench scores are shown for reference; Overall is reported only when all benchmarks are available; cells marked \texttt{--} are reserved for newly added baselines, AgentDoG~2.0 retraining, and ATBench-Pro evaluation.}
  \label{tab:agentdog2-fine}
\end{table*}

\begin{figure*}[h]
  \centering
  \fbox{\parbox{0.9\linewidth}{\centering
    \vspace{2em}
    \textbf{PLACEHOLDER:} fine-grained risk diagnosis accuracy versus inference efficiency.\\
    To be populated after the final evaluation.
    \vspace{2em}}}
  \caption{\textbf{Placeholder:} fine-grained risk diagnosis accuracy versus inference efficiency.}
\end{figure*}

\subsubsection{Inference Efficiency and Pareto Frontier}
% TODO: Fill in inference efficiency and Pareto frontier analysis (Table~\ref{tab:agentdog2-efficiency}, figure placeholders).

\begin{table*}[h]
  \centering
  \small
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}lccccccccc@{}}
    \toprule
    & \multicolumn{3}{c}{\textbf{R-Judge Factor ($\times$)}}
      & \multicolumn{3}{c}{\textbf{ATBench Factor ($\times$)}}
      & \multicolumn{3}{c}{\textbf{ATBench-Pro Factor ($\times$)}} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(l){8-10}
    \textbf{Base Model} & Out. & Tot. & Lat.
      & Out. & Tot. & Lat.
      & Out. & Tot. & Lat. \\
    \midrule
    Qwen3.5-0.8B  & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Qwen3.5-2B    & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Qwen3.5-4B    & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Llama-3.1-8B  & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Qwen3.5-9B    & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Inference efficiency gains of AgentDoG~2.0 relative to AgentDoG~1.5-U across base models.}
    Each factor ($\times$) equals the AgentDoG~1.5-U value divided by the AgentDoG~2.0 value for output tokens (Out.), total tokens (Tot.), and mean wall-clock latency (Lat.).}
  \label{tab:agentdog2-efficiency}
\end{table*}

==> sections/agentdog_jev.tex <==
\section{\agentdogjev{}}
\label{sec:agentdog-jev}
% Writing: 李欣皓、马嘉晨
% Review: 刘东瑞
\agentdogjev{} explores a decision-centric architecture for efficient trajectory-level safety evaluation and fine-grained risk diagnosis, aiming to further reduce the inference overhead of agent safety guardrails. 
Building upon AgentDoG 1.5 and following the efficiency-oriented direction of AgentDoG 2.0, \agentdogjev{} draws inspiration from Jev, a System One model introduced by TypeSafe AI for fast and structured decision-making. 
Unlike conventional language models that generate outputs sequentially as text tokens, Jev produces type-safe structured decisions through parallel sampling. 
Inspired by this paradigm, \agentdogjev{} adopts structured decision representations and autoregressive masking to predict safety decisions within a single forward pass, avoiding sequential autoregressive decoding of individual decision fields. 
This design aims to reduce decoding overhead while preserving trajectory-level safety detection capability. 
For the Unified-4B variant on ATBench, \agentdogjev{} achieves a \textbf{109.0$\times$} end-to-end latency speedup over AgentDoG 1.5-U, while retaining \textbf{98.7\%} of its accuracy and \textbf{99.1\%} of its Macro-F1, demonstrating the potential of decision-centric modeling for efficient agent safety evaluation.
\mbox{}

\begin{figure*}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/agentdog-jev-inference-flow.pdf}
    \caption{Overview of the \agentdogjev{} decision pipeline. An input trajectory with a three-field decision schema are processed by the model in one forward pass. The model reads the logits at the three decision positions, and the resulting confidence distributions for failure mode, real world harm, and risk source yield the final diagnosis.}
    \label{fig:jev_pipeline}
\end{figure*}


\subsection{Task Definition}
\label{subsec:agentdog-jev-1}
% Replace the empty line below with manuscript text.
Given an agent trajectory, \agentdogjev{} performs trajectory-level safety evaluation and fine-grained risk diagnosis through structured decision-making. 
The evaluator takes as input $x=(q,\mathcal{U},\tau)$, where $q$ denotes the evaluation instruction, $\mathcal{U}$ represents the set of available tools, and $\tau=(u,s_1,\ldots,s_n)$ denotes the agent trajectory, with $u$ being the initial user request and each step $s_i=(a_i,o_i)$ consisting of an agent action and its corresponding observation. 
Instead of generating free-form reasoning, \agentdogjev{} produces predictions under a fixed output schema, with each decision field associated with a normalized confidence distribution over its candidate labels.

\subsubsection{Structured Decision Formulation}

Let $\mathcal{J}$ denote the set of decision fields, and $\mathcal{C}_j$ denote the candidate label set for field $j\in\mathcal{J}$. During a single forward pass, the model produces logits for all decision fields:
\begin{equation}
\mathbf{L}(x)=
\left\{
\ell_{j,c}(x)
\mid j\in\mathcal{J},\ c\in\mathcal{C}_j
\right\},
\end{equation}
where $\ell_{j,c}(x)$ denotes the logit associated with candidate $c$ in field $j$.

At inference time, a normalized confidence distribution is obtained by applying softmax exclusively over the legal candidate tokens of each field:
\begin{equation}
p_j(c\mid x)=
\frac{\exp(\ell_{j,c}(x))}
{\displaystyle\sum_{c'\in\mathcal{C}_j}
\exp(\ell_{j,c'}(x))}.
\end{equation}
The predicted label and its associated confidence are:
\begin{equation}
\hat{y}_j=
\arg\max_{c\in\mathcal{C}_j}p_j(c\mid x),
\qquad
\hat{p}_j=p_j(\hat{y}_j\mid x).
\end{equation}
All field logits are obtained from the same forward pass, without separate field-wise forward passes, prediction backfilling, or intermediate Chain-of-Thought (CoT) generation.

\subsubsection{Trajectory-level Safety}

The first task determines whether an agent trajectory contains unsafe behavior. Its candidate label set is:
\begin{equation}
\mathcal{C}_{\mathrm{safe}}=
\{\texttt{safe},\texttt{unsafe}\}.
\end{equation}
The predicted safety label is:
\begin{equation}
\hat{z}=
\arg\max_{c\in\mathcal{C}_{\mathrm{safe}}}
p_{\mathrm{safe}}(c\mid x).
\end{equation}
A trajectory is classified as unsafe if at least one agent action or decision violates safety requirements or leads to potentially harmful behavior. Conversely, a trajectory is considered safe if the agent handles the user's request appropriately, including safely rejecting or handling potentially harmful requests.

\subsubsection{Fine-grained Risk Diagnosis}

Beyond binary safety classification, \agentdogjev{} characterizes unsafe behaviors through three complementary dimensions: \textit{Risk Source}, \textit{Failure Mode}, and \textit{Real-world Harm}. Let their respective candidate label sets be $\mathcal{C}_{\mathrm{source}}$, $\mathcal{C}_{\mathrm{failure}}$, and $\mathcal{C}_{\mathrm{harm}}$, as defined by the safety risk taxonomy. For an unsafe trajectory, the model predicts:
\begin{equation}
\hat{\mathbf{y}}=
(\hat{y}_{\mathrm{source}},
\hat{y}_{\mathrm{failure}},
\hat{y}_{\mathrm{harm}}),
\end{equation}
where each label is selected according to the highest normalized confidence:
\begin{equation}
\hat{y}_{j}=
\arg\max_{c\in\mathcal{C}_{j}}p_j(c\mid x),
\quad
j\in\{\mathrm{source},\mathrm{failure},\mathrm{harm}\}.
\end{equation}
Each predicted diagnosis is accompanied by its confidence score, identifying where the risk originates, how the agent fails, and what potential real-world consequences may arise.

\mbox{}

\subsection{Data Preparation}
\label{subsec:agentdog-jev-2}

\begin{figure*}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/agentdog-jev-prompt-template.pdf}
    \caption{The trajectory-level safety and fine-grained risk diagnosis prompt templates adopted by \agentdogjev{}. Both templates define explicit decision schemas and corresponding candidate symbols, with the assistant targets formatted as structured JSON outputs.}
    \label{fig:jev_prompt_templates}
\end{figure*}

\agentdogjev{} constructs two SFT datasets for trajectory-level safety classification and fine-grained risk diagnosis based on the original AgentDoG 1.5 SFT dataset. We retain the original agent trajectories and supervision labels while adapting the input and target formats to support decision-centric learning. Specifically, we construct two task-specific datasets using the prompt templates illustrated in Figure~\ref{fig:jev_prompt_templates}.

For trajectory-level safety classification, each sample is paired with a binary safety label, represented by one of two candidate symbols corresponding to \textit{safe} and \textit{unsafe}. For fine-grained risk diagnosis, each sample is paired with a structured label tuple covering three dimensions: \textit{Risk Source}, \textit{Failure Mode}, and \textit{Real-world Harm}. The corresponding candidate symbol sets contain 8, 14, and 10 categories, respectively. Each candidate category is assigned a unique single-token symbol, enabling direct decision scoring without aggregating logits across multiple tokens.

The resulting datasets are formally defined as:
\begin{equation}
\begin{aligned}
\mathcal{D}_{\mathrm{traj}}
&=
\{(x_i,y_i^{\mathrm{traj}})\}_{i=1}^{N_{\mathrm{traj}}},\\
\mathcal{D}_{\mathrm{FG}}
&=
\{(x_j,\mathbf{y}_j^{\mathrm{FG}})\}_{j=1}^{N_{\mathrm{FG}}},
\end{aligned}
\end{equation}
where $x=(q,\mathcal{U},\tau)$ denotes the task-specific input, including the evaluation instruction, available tools, and complete agent trajectory. The rajectory-level target $y_i^{\mathrm{traj}}$ represents the binary safety decision, while the fine-grained target tuple is defined as
\begin{equation}
\mathbf{y}_j^{\mathrm{FG}}
=
(y_j^{\mathrm{source}},
y_j^{\mathrm{failure}},
y_j^{\mathrm{harm}}).
\end{equation}

For both tasks, the assistant targets are formatted as structured JSON output skeletons, with each decision field replaced by a special \texttt{<decision>} token during training. The corresponding target symbols provide supervision at these positions, while no CoT rationale or intermediate textual analysis is included in the supervised outputs. This formulation enables the model to learn binary safety decisions and multi-dimensional risk diagnoses through the same decision-oriented training mechanism.
\mbox{}


\subsection{Training}
\label{subsec:agentdog-jev-3}

\agentdogjev{} is trained through supervised fine-tuning (SFT), initialized from the pretrained AgentDoG 1.5 model checkpoint rather than its original foundation model. During training, supervision is applied exclusively to the \texttt{<decision>} positions, while all remaining tokens are masked out from loss computation. Under causal attention, the logits at the position immediately preceding each \texttt{<decision>} token are used to predict its corresponding target symbol through full-vocabulary cross-entropy.

\textbf{Trajectory-level Safety SFT.} For binary safety classification, each sample contains a single \texttt{<decision>} position, supervised with one of two target symbols representing \textit{safe} and \textit{unsafe}. Given the training dataset $\mathcal{D}_{\mathrm{traj}}$, the objective is defined as:

\begin{equation}
\mathcal{L}_{\mathrm{traj}}(\theta)
=
-\mathbb{E}_{(x,y)\sim\mathcal{D}_{\mathrm{traj}}}
\log \pi_\theta(y\mid x,p-1),
\end{equation}

where $p$ denotes the position of the \texttt{<decision>} token, and the target symbol is predicted using the logits at position $p-1$ under the causal language modeling objective.

\textbf{Fine-grained Risk Diagnosis SFT.} For fine-grained diagnosis, three \texttt{<decision>} positions correspond to \textit{Risk Source}, \textit{Failure Mode}, and \textit{Real-world Harm}, respectively. Their losses are jointly optimized within a single forward pass. Given the training dataset $\mathcal{D}_{\mathrm{FG}}$, the joint objective is:

\begin{equation}
\mathcal{L}_{\mathrm{FG}}(\theta)
=
-\mathbb{E}_{(x,y)\sim\mathcal{D}_{\mathrm{FG}}}
\frac{1}{F}
\sum_{k=1}^{F}
\log \pi_\theta(y_k\mid x,p_k-1),
\qquad F=3,
\end{equation}

where $p_k$ and $y_k$ denote the decision position and target symbol of field $k$, respectively. All three diagnosis fields are available for every training sample. Their target symbols cover 14 Failure Mode categories, 10 Real-world Harm categories, and 8 Risk Source categories. Thus, fine-grained training extends the single-position objective to three jointly supervised decision positions.

Both training tasks use two epochs with a learning rate of $2\times10^{-6}$. At inference time, the model applies softmax exclusively over the valid candidate symbols of each field to obtain normalized decision confidence scores, avoiding the need for autoregressive generation of the structured output.
\mbox{}

\subsection{Evaluation}
\label{subsec:agentdog-jev-4}
\subsubsection{Experimental Setup}

\paragraph{Models and baselines.}
For trajectory-level safety judgment, we evaluate five AgentDoG~1.5 checkpoints built on Qwen3.5-0.8B, Qwen3.5-2B, Qwen3.5-4B, the unified 4B model, and Llama-3.1-8B. We train the corresponding \agentdogjev{} decision heads and compare them with the original generative AgentDoG~1.5 models, which produce CoT analysis followed by a \texttt{safe/unsafe} verdict.
For fine-grained risk diagnosis, we evaluate four AgentDoG~1.5 Fine-Grained checkpoints: FG-Qwen-0.8B, FG-Qwen-2B, FG-Qwen-4B, and FG-Llama-8B. Each checkpoint is compared with its corresponding \agentdogjev{} variant and generative baseline, which produces an analysis followed by the three diagnostic labels.

In addition to these AgentDoG-based models, we include five open-source models (Qwen3.5-0.8B, Qwen3.5-2B, Qwen3.5-4B, Qwen3.5-9B, and Llama-3.1-8B) as reference points in the Pareto plots. These models provide additional reference points for comparing the efficiency--performance trade-offs of \agentdogjev{} against standalone open-source models.

\paragraph{Benchmarks and metrics.}
We evaluate coarse-grained models on ATBench and R-Judge and report Accuracy and Macro-F1.
Fine-grained models are evaluated on the 497 gold-unsafe ATBench trajectories that carry valid labels in all three dimensions.
We report accuracy for risk source, failure mode, and real-world harm, and use their mean as the aggregate diagnostic accuracy.
All \agentdogjev{} predictions are obtained by taking the argmax over the legal candidate tokens of each field, so they are always valid labels; baseline outputs are parsed from generated text.
Re-evaluating the official fine-grained checkpoints on the same 497 trajectories reproduces the averages reported by AgentDoG~1.5 within 1.5 points on average, which places the comparison on a consistent footing.

\paragraph{Efficiency measures.}
We adopt the same end-to-end latency measurement protocol as \agentdog{} (Section~\ref{subsec:agentdog-4}).
Each method is timed with its native prompt and output procedure: single-prefill decision readout for \agentdogjev{} and autoregressive decoding for the baselines.

\begin{table*}[h]
  \centering
  \caption{\textbf{Trajectory-level safety judgment on ATBench and R-Judge.}
    Accuracy and Macro-F1 are percentages formatted as AgentDoG~1.5 baseline $\to$ \agentdogjev{}, with bold marking an improvement over the baseline.
    Mean latency (seconds) and speedup are averaged over all timing requests; speedup is the baseline-to-\agentdogjev{} ratio.}
  \label{tab:jev-coarse-performance}
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{Macro-F1}
      & \multirow{2}{*}{Latency (s) $\downarrow$} & \multirow{2}{*}{Speedup $\uparrow$} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}
    Base Model & ATBench & R-Judge & ATBench & R-Judge & & \\
    \midrule
    Qwen3.5-0.8B & 62.90 $\to$ 51.20 & 78.55 $\to$ \textbf{80.32}
                 & 61.80 $\to$ 42.30 & 78.09 $\to$ \textbf{80.27}
                 & 7.03 $\to$ 0.038 & 184.9$\times$ \\
    Qwen3.5-2B   & 63.70 $\to$ 63.70 & 87.23 $\to$ 85.46
                 & 62.00 $\to$ 61.70 & 87.21 $\to$ 85.42
                 & 7.04 $\to$ 0.040 & 176.5$\times$ \\
    Qwen3.5-4B   & 69.30 $\to$ 69.00 & 88.83 $\to$ 86.35
                 & 69.10 $\to$ 68.90 & 88.78 $\to$ 86.20
                 & 9.18 $\to$ 0.059 & 155.8$\times$ \\
    Unified-4B   & 78.10 $\to$ 77.10 & 90.78 $\to$ 81.91
                 & 77.80 $\to$ 77.10 & 90.78 $\to$ 81.50
                 & 6.52 $\to$ 0.060 & 109.0$\times$ \\
    Llama-3.1-8B & 64.90 $\to$ \textbf{66.20} & 86.35 $\to$ 75.35
                 & 64.10 $\to$ \textbf{64.30} & 86.21 $\to$ 73.81
                 & 5.10 $\to$ 0.049 & 103.9$\times$ \\
    \bottomrule
  \end{tabular}
\end{table*}

\subsubsection{Binary Safety Judgment}

\textbf{Across all five checkpoints, \agentdogjev{} reduces end-to-end latency by two orders of magnitude.}
Speedups range from 103.9$\times$ to 184.9$\times$ (Table~\ref{tab:jev-coarse-performance}), with all models achieving sub-0.1s inference latency. This substantial reduction stems from replacing autoregressive decoding with a single prefill followed by decision-position readout. In contrast, the generative baselines produce 316--591 output tokens before reaching a safety verdict. Consequently, \agentdogjev{} maintains nearly constant inference latency across model scales, while the speedup varies primarily with the decoding overhead of each baseline.

\textbf{Most checkpoints preserve the baseline's safety performance, with two instructive exceptions.}
On ATBench, the 2B, 4B, and unified-4B models exhibit only marginal performance differences from their generative counterparts, with the unified-4B model retaining 98.7\% of accuracy and 99.1\% of Macro-F1. The 2B and 4B models also maintain relatively close performance on R-Judge, suggesting that decision-centric prediction can preserve much of the original model's trajectory-level safety evaluation capability without generating explicit reasoning. However, the performance differences across benchmarks indicate that this capability remains sensitive to the evaluation data and underlying model representations.

\textbf{The 0.8B checkpoint exhibits a pronounced performance drop on ATBench despite improving on R-Judge.}
Its ATBench accuracy and Macro-F1 decrease substantially, whereas both metrics improve on R-Judge. One possible explanation is that the longer trajectories in ATBench impose greater demands on the model's ability to retain and integrate safety-relevant evidence across the full context. With limited model capacity, the decision head may struggle to distinguish relevant evidence from the surrounding trajectory and rely more heavily on learned decision priors. The better results on R-Judge suggest that this limitation is not universal, but may become more pronounced under longer or more complex trajectory inputs.

\textbf{Llama-3.1-8B shows the opposite pattern, slightly outperforming its generative baseline on ATBench.}
It improves both accuracy and Macro-F1, indicating that a sufficiently capable backbone can preserve or even improve binary safety discrimination under the decision-centric formulation. This result further suggests that the effectiveness of \agentdogjev{} depends not only on the removal of autoregressive decoding, but also on the backbone's ability to encode trajectory-level safety information into representations accessible at the decision positions.

\begin{figure*}[t]
  \centering
  \IfFileExists{figures/pareto-jev-coarse.pdf}{%
    \includegraphics[width=0.9\linewidth]{figures/pareto-jev-coarse.pdf}%
  }{%
    \fbox{\parbox[c][3.5cm][c]{0.82\linewidth}{\centering\small
      Pareto front placeholder: ATBench Macro-F1 vs.\ mean latency (data pending).}}%
  }
  \caption{\textbf{ATBench and R-Judgesafety Macro-F1 versus mean latency.}
    Points include the AgentDoG~1.5 baselines, the corresponding \agentdogjev{} decision models and five open-source models as reference points.
    Dashed lines connect Pareto-optimal points.
    Latency is the mean end-to-end request latency over all timing requests;
    higher scores at lower latency are preferable.}
  \label{fig:jev-pareto-coarse}
\end{figure*}

\textbf{The Pareto Frontier plots further demonstrate the efficiency advantage of AgentDoG-Jev across both benchmarks.} 
As shown in Figure~\ref{fig:jev-pareto-coarse}, AgentDoG-Jev on ATBench shifts the models toward a substantially lower-latency region while retaining competitive Macro-F1 scores. In particular, the 4B and unified-4B variants achieve relatively strong performance at approximately 0.06s, with the latter reaching 77.1\% Macro-F1. A similar trend is observed on R-Judge, where AgentDoG-Jev achieves Macro-F1 scores of 73.81–86.20\% at only 0.038–0.060s. Compared with the corresponding generative baselines, these results establish a substantially more favorable efficiency–performance trade-off, while the differences between the two benchmarks highlight the influence of evaluation data on the resulting frontier.

\subsubsection{Fine-Grained Risk Diagnosis}

\begin{table*}[h]
  \centering
  \caption{\textbf{Fine-grained risk diagnosis on ATBench.}
    Accuracy is reported on the 497 gold-unsafe trajectories with valid labels in all three dimensions, formatted as AgentDoG~1.5 Fine-Grained baseline $\to$ \agentdogjev{}; bold marks a higher accuracy than the baseline.
    Average is the mean of the three field accuracies.
    Mean latency (seconds) and speedup are averaged over all timing requests; speedup is the baseline-to-\agentdogjev{} ratio.}
  \label{tab:jev-fine-performance}
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{4}{c}{Diagnostic Accuracy (\%) $\uparrow$}
      & \multicolumn{2}{c}{Efficiency} \\
    \cmidrule(lr){2-5}\cmidrule(l){6-7}
    Base Model & Risk Source & Failure Mode & Real-world Harm & Average
      & Latency (s) $\downarrow$ & Speedup $\uparrow$ \\
    \midrule
    FG-Qwen-0.8B & 61.57 $\to$ 56.14 & 21.33 $\to$ 20.32 & 48.69 $\to$ \textbf{51.31}
                 & 43.86 $\to$ 42.59 & 3.218 $\to$ 0.358 & 8.99$\times$ \\
    FG-Qwen-2B   & 67.81 $\to$ 61.57 & 24.14 $\to$ 23.14 & 53.92 $\to$ \textbf{56.54}
                 & 48.63 $\to$ 47.08 & 4.335 $\to$ 0.341 & 12.7$\times$ \\
    FG-Qwen-4B   & 71.43 $\to$ 63.38 & 27.16 $\to$ \textbf{28.77} & 62.58 $\to$ 59.96
                 & 53.72 $\to$ 50.70 & 4.749 $\to$ 0.355 & 13.4$\times$ \\
    FG-Llama-8B  & 67.40 $\to$ 63.38 & 21.53 $\to$ \textbf{28.37} & 50.30 $\to$ \textbf{56.74}
                 & 46.41 $\to$ \textbf{49.50} & 1.606 $\to$ 0.364 & 4.4$\times$ \\
    \bottomrule
  \end{tabular}
\end{table*}

\textbf{Across the four fine-grained checkpoints, \agentdogjev{} reduces end-to-end latency by 1.6--13.4$\times$.}
The largest gains are observed on the 2B and 4B models, while Llama-3.1-8B achieves a 4.4$\times$ speedup (Table~\ref{tab:jev-fine-performance}). Despite differences in model scale and baseline generation length, \agentdogjev{} maintains a relatively stable latency of 0.341--0.364s across all four checkpoints. This consistency reflects the removal of most autoregressive decoding overhead, whereas the varying speedups are primarily determined by how much analysis the corresponding generative baselines produce.

\textbf{Risk-source accuracy decreases across all four checkpoints, whereas failure-mode and real-world-harm accuracy show model-dependent changes.} 
This may reflect the greater difficulty of risk-source attribution, which requires tracing unsafe behavior back to potentially earlier user instructions, tool descriptions, or tool outputs across the trajectory. While generative baselines can explicitly establish these relationships through intermediate analysis, AgentDoG-Jev must encode them directly into decision representations within a single forward pass. By contrast, failure mode and real-world harm are more closely associated with executed actions and their observed consequences, making them potentially easier to recover from trajectory representations. This is reflected in the improvements on selected checkpoints, particularly for failure-mode accuracy on 4B and Llama-8B, and real-world-harm accuracy on 0.8B, 2B, and Llama-8B. Nevertheless, failure mode remains the most challenging dimension, with accuracy ranging from 20.32\% to 28.77\%, highlighting the difficulty of fine-grained diagnosis despite substantially reduced inference overhead.

\textbf{Llama-3.1-8B is the only checkpoint that improves overall diagnostic accuracy.}
Its average accuracy increases from 46.41\% to 49.50\%, as improvements in failure mode and real-world harm outweigh the decline in risk-source accuracy. In contrast, the other three checkpoints experience modest reductions in average accuracy. The 4B model exhibits the largest decline because its substantial loss in risk-source accuracy is accompanied by a decrease in real-world-harm accuracy, which cannot be offset by its relatively small improvement in failure mode. These results suggest that the effectiveness of decision-centric diagnosis depends on how well each backbone represents the different dimensions of risk, rather than producing uniform improvements across all diagnostic fields.

\begin{figure*}[t]
  \centering
  \IfFileExists{figures/pareto-jev-atbench-fine.pdf}{%
    \includegraphics[width=0.8\linewidth]{figures/pareto-jev-atbench-fine.pdf}%
  }{%
    \fbox{\parbox[c][3.5cm][c]{0.82\linewidth}{\centering\small
      Pareto front placeholder: ATBench fine-grained average accuracy vs.\ mean latency (data pending).}}%
  }
  \caption{\textbf{ATBench fine-grained diagnostic accuracy versus mean latency.}
    Points include the four AgentDoG~1.5 Fine-Grained baselines, their \agentdogjev{} counterparts and five open-source models as reference points.
    Dashed lines connect Pareto-optimal points.
    Accuracy is the mean of risk-source, failure-mode, and real-world-harm accuracy.
    Latency is the mean end-to-end request latency over all timing requests.}
  \label{fig:jev-pareto-atbench-fine}
\end{figure*}

\textbf{The fine-grained Pareto Frontier plot shows that AgentDoG-Jev substantially improves inference efficiency while retaining competitive diagnostic accuracy.} 
As shown in Figure~\ref{fig:jev-pareto-atbench-fine}, all four AgentDoG-Jev models operate within a narrow latency range of 0.341–0.364s, compared with 1.606–4.749s for their generative baselines. Among them, FG-Qwen-4B achieves the highest average diagnostic accuracy of 50.70\% at 0.355s, while FG-Llama-8B improves over its baseline in both latency and average accuracy, reaching 49.50\% at 0.364s. The 2B and 4B variants also provide substantial latency reductions with relatively limited accuracy trade-offs. Overall, the results show that decision-centric inference moves fine-grained diagnosis toward a more favorable efficiency–accuracy region, although the extent of accuracy retention remains backbone-dependent.
\mbox{}



==> sections/agentdog_step.tex <==
\section{\agentdogstep{}}
\label{sec:agentdog-step}
% Writing: 段东杭、马嘉晨、李宇
% Review: 王鹏
AgentDoG-Step extends our diagnostic to the pre-execution step boundary, judging each candidate tool call or response strictly from the prior interaction prefix.
Across TS-Bench and StepShield, lightweight AgentDoG-Step models achieve the strongest overall balance between blocking unsafe actions and preserving benign workflows, outperforming dedicated safety guards as well as substantially larger general-purpose LLMs.

\subsection{Task Definition}
\label{subsec:agentdog-step-task}
Following the trajectory-level formulation in Section~\ref{subsec:agentdog-1}, we adapt safety evaluation and fine-grained diagnosis to the pre-execution step boundary.
Let $\mathcal{T}_{<i}=(u,t_1,\ldots,t_{i-1})$ denote the interaction prefix through step $i-1$, where $u$ is the initial user request and each completed step $t_j=(a_j,o_j)$ pairs an earlier agent action $a_j$ with its environment observation $o_j$.
Given the pre-execution input
\begin{equation}
  x_i = (q,\mathcal{U},\mathcal{T}_{<i},a_i),
\end{equation}
where $q$ specifies the evaluation instruction, $\mathcal{U}$ denotes the available tool descriptions, and $a_i$ is the candidate action at step~$i$, the guard evaluates $a_i$ before it is executed or delivered to the user.
The resulting observation $o_i$ and all subsequent steps remain strictly outside $x_i$.

\paragraph{Step-level safety and fine-grained diagnosis.}
The binary safety judgment $y_i \in \{\texttt{safe}, \texttt{unsafe}\}$ satisfies
\begin{equation}
  y_i = \texttt{unsafe}
  \quad\Longleftrightarrow\quad
  \mathsf{Unsafe}(\mathcal{T}_{<i},a_i) = \mathrm{True},
\end{equation}
where $\mathsf{Unsafe}(\cdot)$ assesses $a_i$ conditioned solely on the visible pre-execution context; appropriately refusing or safely handling a risky request or observation still yields a \texttt{safe} judgment.
Using the same three-dimensional taxonomy label spaces ($\ell_i^{\text{mode}}\in\mathcal{L}^{\text{mode}}$, $\ell_i^{\text{harm}}\in\mathcal{L}^{\text{harm}}$, and $\ell_i^{\text{risk}}\in\mathcal{L}^{\text{risk}}\cup\{\texttt{None}\}$), the step-level target tuple is
\begin{equation}
  y_{\mathrm{fine},i} =
  \begin{cases}
    (y_i, \ell_i^{\text{risk}}), & y_i = \texttt{safe},\\
    (y_i, \ell_i^{\text{mode}}, \ell_i^{\text{harm}}, \ell_i^{\text{risk}}), & y_i = \texttt{unsafe}.
  \end{cases}
\end{equation}
Decoupling the risk origin ($\ell_i^{\text{risk}}$) from unsafe realization ($\ell_i^{\text{mode}}, \ell_i^{\text{harm}}$) allows a safe step to carry a non-\texttt{None} $\ell_i^{\text{risk}}$ when the agent safely navigates a risky context.

\paragraph{Evidence-grounded rationale.}
Conditioned on $x_i$, AgentDoG-Step first emits a brief \texttt{<Analysis>} rationale grounded strictly in the visible prefix and candidate action, followed by a serialized response $r_i$ containing the named fields of $y_{\mathrm{fine},i}$.
Retaining a concise rationale stabilizes boundary decisions under partial pre-execution visibility---helping distinguish benign handling of risky contexts from genuinely unsafe execution---while providing an auditable justification whenever an action is blocked.

%%%%%

\subsection{Data Preparation}
\label{subsec:agentdog-step-2}
% TODO: Fill in Data Preparation.
\mbox{}

%%%%%

\subsection{Training}
\label{subsec:agentdog-step-3}
We adopt the same two-stage SFT and GDPO training pipeline introduced in Section~\ref{subsec:agentdog-3}, adapting the supervision format and RL regularization to pre-execution step guarding.

\subsubsection{Supervised Fine-Tuning}
Using the token-level negative log-likelihood objective $\mathcal{L}_{\mathrm{SFT}}(\theta)$ in Section~\ref{subsec:agentdog-3} with prompt tokens masked, we fine-tune the base model on pre-execution demonstrations $(x_i,r_i)\sim\mathcal{D}_{\mathrm{SFT}}$, where $r_i$ pairs the brief \texttt{<Analysis>} block with the serialized step diagnosis $y_{\mathrm{fine},i}$.
We train for $3$ epochs in \texttt{bf16} using AdamW (weight decay $0$, gradient norm clipping $1.0$), a peak learning rate of $2\times 10^{-5}$ with a cosine schedule and $10\%$ warmup, a maximum sequence length of $16{,}384$, and a per-device batch size of $1$ with $16$ gradient accumulation steps.

\subsubsection{Reinforcement Learning}
Starting from the SFT checkpoint, we optimize the policy $\pi_\theta$ using the GDPO group-normalized clipped surrogate formulation in Section~\ref{subsec:agentdog-3}, augmented with a KL penalty ($\beta = 10^{-3}$) against the frozen SFT reference policy $\pi_{\mathrm{ref}}$ to prevent drift from the SFT reasoning distribution.
For each pre-execution query $x_i$, a deterministic verifier scores each applicable field $k\in\mathcal{K}_i$ with a binary exact-match reward $\rho_{i,j,k}\in\{0,1\}$ (with format-invalid completions receiving zero across all fields):
\begin{equation}
  \mathcal{K}_i =
  \begin{cases}
    \{\mathrm{Safety},\mathrm{RS}\}, & y_i^*=\texttt{safe},\\
    \{\mathrm{Safety},\mathrm{RS},\mathrm{FM},\mathrm{RWH}\}, & y_i^*=\texttt{unsafe}.
  \end{cases}
\end{equation}
For gold-unsafe steps, fine-grained fields ($\mathrm{RS}, \mathrm{FM}, \mathrm{RWH}$) receive credit only when the completion also predicts $\hat{y}_{i,j}=\texttt{unsafe}$.
For gold-safe steps, including $\mathrm{RS}$ in $\mathcal{K}_i$ awards Risk Source credit independently of the binary judgment.
Under variance-filtered GDPO, this mitigates the reward-variance asymmetry between safe and unsafe rollout groups: safe groups with unanimous binary Safety predictions still qualify for policy updates whenever their Risk Source attributions vary.
We train for $200$ RL iterations using Adam ($\beta_1=0.9$, $\beta_2=0.98$, weight decay $0.1$, gradient clipping $1.0$), a constant learning rate of $1\times 10^{-6}$, clip bounds $(\epsilon_{\mathrm{low}},\epsilon_{\mathrm{high}})=(0.2,0.28)$, rollout temperature $1.0$, $G=8$ rollouts per query, and a global batch size of $128$.

%%%%%

\subsection{Evaluation}
\label{subsec:agentdog-step-4}

\subsubsection{Experimental Setup}

\paragraph{Models and baselines.}
We evaluate five AgentDoG-Step variants initialized from Qwen3.5 (0.8B, 2B, 4B, and 9B) and Llama-3.1-8B.
Baselines span three groups: closed-source frontier models (GPT-6.1-Sol, GPT-5.4, and Gemini~3.8 Flash), open-weight general models from the Qwen and Llama families, and three dedicated safety guards (Qwen3Guard-8B, LlamaGuard-8B, and StepGuard~\citep{zheng2026stepguard}).

\paragraph{Benchmarks and protocol.}
Because existing public step-level benchmarks provide only binary safety labels, we evaluate pre-execution binary step-level safety on TS-Bench-Dojo ($1{,}220$ steps), TS-Bench-ASB ($3{,}765$ steps)~\citep{mou2026toolsafe}, and StepShield ($2{,}670$ steps)~\citep{stepshield2026}.
All guards observe strictly the pre-execution prefix and candidate action, while post-action benchmark annotations serve as ground truth.
Dedicated guards use their native moderation interfaces or templates, whereas all remaining models use our step-level diagnosis template.

\paragraph{Metrics.}
Alongside accuracy and unsafe-class F1, we report worst-class recall (WCR) to evaluate the balance between safe-action preservation and unsafe-action interception:
\begin{equation}
  \mathrm{WCR} = \min\{\mathrm{Recall}_{\mathrm{Safe}}, \mathrm{Recall}_{\mathrm{Unsafe}}\}.
\end{equation}
\textsc{Overall} reports the unweighted mean across the three benchmarks.
For the controlled ablation on TS-Bench-Dojo, we additionally report safe-class F1.

\begin{table*}[h]
  \centering
  \begingroup
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.1}
  \definecolor{agentdogstepsection}{HTML}{EBD3AC}
  \definecolor{agentdogsteprank1}{HTML}{98CE9B}
  \definecolor{agentdogsteprank2}{HTML}{AED8B0}
  \definecolor{agentdogsteprank3}{HTML}{C5E3C6}
  \newcommand{\agentdogstepranked}[2]{\cellcolor{agentdogsteprank#1}\ifnum#1=1 \textbf{#2}\else #2\fi}
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{l*{12}{>{\centering\arraybackslash}p{1.25cm}}}
      \toprule
      \textbf{Model}
       & \multicolumn{3}{c}{\textbf{TS-Bench-Dojo}}
       & \multicolumn{3}{c}{\textbf{TS-Bench-ASB}}
       & \multicolumn{3}{c}{\textbf{StepShield}}
       & \multicolumn{3}{c}{\textbf{Overall}} \\
      \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
       & Acc $\uparrow$ & F1 $\uparrow$ & WCR $\uparrow$
         & Acc $\uparrow$ & F1 $\uparrow$ & WCR $\uparrow$
         & Acc $\uparrow$ & F1 $\uparrow$ & WCR $\uparrow$
         & Acc $\uparrow$ & F1 $\uparrow$ & WCR $\uparrow$ \\
      \midrule
      \rowcolor{agentdogstepsection}\multicolumn{13}{l}{\textbf{Closed-Source Models}} \\
      GPT-6.1-Sol & 96.9 & 94.9 & 96.4 & 69.2 & 55.0 & 66.3 & 85.4 & 35.5 & 84.9 & 83.8 & 61.8 & 82.5 \\
      GPT-5.4 & 96.8 & 94.7 & 95.9 & 78.5 & 66.1 & 73.6 & 89.8 & 44.0 & 89.4 & 88.4 & 68.3 & 86.3 \\
      Gemini~3.8 Flash & 97.7 & 97.0 & 97.7 & 91.0 & 87.4 & 87.8 & 95.9 & 71.6 & 94.4 & 94.9 & 85.4 & 93.3 \\
      Gemini~3.1 Pro & 96.7 & 94.5 & 96.3 & 80.6 & 74.1 & 73.6 & 88.5 & 41.2 & 88.1 & 88.6 & 69.9 & 86.0 \\
      \addlinespace[2.5pt]
      \rowcolor{agentdogstepsection}\multicolumn{13}{l}{\textbf{Open-Source Models}} \\
      Qwen3.5-397B & 91.6 & 87.3 & 88.6 & 76.2 & 64.9 & \agentdogstepranked{2}{75.8} & 95.6 & 64.9 & 95.5 & 87.8 & 72.3 & 86.6 \\
      Qwen3-235B & 93.4 & 89.6 & 91.7 & 78.6 & 51.6 & 40.1 & 98.7 & 86.3 & \agentdogstepranked{2}{98.7} & 90.3 & 75.8 & 76.9 \\
      Qwen3.8-27B & 95.5 & 92.7 & 94.2 & 78.4 & 64.1 & 67.9 & 96.1 & 67.3 & 96.0 & 90.0 & 74.7 & 86.0 \\
      Qwen3.5-9B & 86.8 & 74.5 & 65.6 & 76.8 & 59.2 & 58.1 & 95.2 & 62.6 & 95.2 & 86.3 & 65.5 & 73.0 \\
      Llama-3.1-8B & 70.9 & 65.0 & 54.3 & 66.7 & 32.4 & 23.4 & 84.9 & 70.1 & 75.9 & 74.2 & 55.8 & 51.2 \\
      Qwen2.5-7B & 76.8 & 37.5 & 24.2 & 73.5 & 28.0 & 18.2 & 98.2 & 75.5 & 68.5 & 82.8 & 47.0 & 36.9 \\
      Qwen3.5-4B & 86.9 & 77.7 & 79.0 & 77.0 & 63.5 & 70.7 & 90.5 & 45.3 & 90.2 & 84.8 & 62.2 & 80.0 \\
      Qwen3-4B & 77.5 & 44.7 & 29.6 & 70.2 & 22.3 & 13.6 & 94.3 & 72.9 & 75.9 & 80.7 & 46.7 & 39.7 \\
      Qwen3.5-0.8B & 71.3 & 17.2 & 10.2 & 70.3 & 36.3 & 29.8 & 96.7 & 59.8 & 59.3 & 79.4 & 37.8 & 33.1 \\
      \addlinespace[2.5pt]
      \rowcolor{agentdogstepsection}\multicolumn{13}{l}{\textbf{Guard Models}} \\
      Qwen3Guard-8B & 71.2 & \phantom{0}0.0 & \phantom{0}0.0 & 73.2 & 13.1 & \phantom{0}7.0 & 98.3 & 73.7 & 58.3 & 80.9 & 28.9 & 21.8 \\
      LlamaGuard-8B & 77.5 & 43.5 & 30.1 & 73.4 & 41.9 & 33.8 & 97.9 & 64.6 & 48.2 & 82.9 & 50.0 & 37.3 \\
      StepGuard & \agentdogstepranked{2}{96.2} & \agentdogstepranked{2}{93.7} & 94.9 & 84.9 & 66.4 & 52.4 & \agentdogstepranked{1}{99.1} & \agentdogstepranked{1}{89.8} & \agentdogstepranked{3}{98.2} & \agentdogstepranked{3}{93.4} & \agentdogstepranked{3}{83.3} & 81.8 \\
      \addlinespace[2.5pt]
      \rowcolor{agentdogstepsection}\multicolumn{13}{l}{\textbf{Our Models}} \\
      AgentDoG-Step 0.8B & 88.0 & 82.1 & 84.9 & 80.4 & 65.6 & 66.0 & 96.5 & 65.7 & 82.4 & 88.3 & 71.1 & 77.8 \\
      AgentDoG-Step 2B & 95.6 & 92.6 & 95.4 & \agentdogstepranked{3}{86.6} & \agentdogstepranked{3}{75.6} & 73.3 & 98.0 & 78.2 & 89.8 & \agentdogstepranked{3}{93.4} & 82.2 & 86.2 \\
      AgentDoG-Step 4B & \agentdogstepranked{2}{96.2} & \agentdogstepranked{3}{93.6} & \agentdogstepranked{2}{95.9} & \agentdogstepranked{1}{89.1} & \agentdogstepranked{1}{82.1} & \agentdogstepranked{1}{87.9} & \agentdogstepranked{2}{98.8} & \agentdogstepranked{3}{86.9} & \agentdogstepranked{3}{98.2} & \agentdogstepranked{1}{94.7} & \agentdogstepranked{1}{87.5} & \agentdogstepranked{1}{94.0} \\
      AgentDoG-Step 8B & 95.8 & 93.0 & \agentdogstepranked{3}{95.7} & \agentdogstepranked{2}{88.5} & \agentdogstepranked{2}{78.8} & 74.9 & 96.8 & 70.6 & 94.4 & \agentdogstepranked{2}{93.7} & 80.8 & \agentdogstepranked{3}{88.4} \\
      AgentDoG-Step 9B & \agentdogstepranked{1}{96.5} & \agentdogstepranked{1}{94.1} & \agentdogstepranked{1}{96.1} & 83.3 & 72.0 & \agentdogstepranked{3}{75.7} & \agentdogstepranked{2}{98.8} & \agentdogstepranked{2}{87.4} & \agentdogstepranked{1}{98.8} & 92.9 & \agentdogstepranked{2}{84.5} & \agentdogstepranked{2}{90.2} \\
      \bottomrule
    \end{tabular}%
  }
  \endgroup
  \caption{\textbf{Pre-execution step-level safety classification across three benchmarks (all scores in \%).}
    AgentDoG-Step 8B is based on Llama-3.1-8B; all other AgentDoG-Step variants use Qwen3.5.
    Green shading marks the top three non-closed-source entries per column (including ties), with boldface indicating the top-ranked non-closed-source model; closed-source models are shown for reference.}
  \label{tab:agentdog-step-main}
\end{table*}

\subsubsection{Binary Safety Judgment}

\paragraph{AgentDoG-Step achieves strong and balanced pre-execution safety judgment.}
As shown in Table~\ref{tab:agentdog-step-main} and illustrated in Figure~\ref{fig:agentdog-step-main}, AgentDoG-Step~4B attains the strongest overall balance across all evaluated models, reaching $94.0\%$ mean WCR and $87.5\%$ unsafe F1.
Despite using only 4B parameters, it surpasses the strongest closed-source baseline, Gemini~3.8 Flash, on both metrics and outperforms frontier open-weight models such as Qwen3.5-397B as well as GPT-5.4 by over $7$ percentage points in overall WCR.

\paragraph{AgentDoG-Step scales effectively across benchmarks and lightweight model sizes.}
As further shown in the per-benchmark breakdown in Figure~\ref{fig:agentdog-step-main}, AgentDoG-Step~9B leads on StepShield and TS-Bench-Dojo, while AgentDoG-Step~4B achieves the highest WCR on the most challenging TS-Bench-ASB split, edging past Gemini~3.8 Flash and outperforming all open-weight baselines by a wide margin.
Lightweight variants retain this favorable balance: AgentDoG-Step~2B matches GPT-5.4 in overall WCR while delivering substantially higher unsafe F1, and AgentDoG-Step~0.8B gains more than $44$ percentage points in overall WCR over its untuned base model.

\paragraph{AgentDoG-Step outperforms dedicated guard baselines.}
Chat-oriented guardrails such as Qwen3Guard-8B and LlamaGuard-8B lose class balance at pre-execution tool-use boundaries, resulting in low WCR across benchmarks.
While StepGuard~\citep{zheng2026stepguard} performs competitively on TS-Bench-Dojo and StepShield, its WCR drops sharply on TS-Bench-ASB, trailing AgentDoG-Step~4B by more than $35$ percentage points on that split and by over $12$ percentage points overall.

\begin{figure*}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figures/step/agentdog-step-main.pdf}
  \caption{\textbf{Pre-execution step-level safety performance of AgentDoG-Step against frontier LLMs and dedicated guards.}
    Panel~(a) plots overall unsafe F1 against overall Worst-Class Recall (WCR), showing that AgentDoG-Step variants occupy the upper-right frontier.
    Panel~(b) compares per-benchmark WCR, highlighting AgentDoG-Step~4B's leading balance on TS-Bench-ASB and overall.}
  \label{fig:agentdog-step-main}
\end{figure*}

\subsubsection{Effect of Safe Risk Source Feedback}
To empirically validate adding Risk Source feedback to safe steps across our framework, we conduct a controlled 4B ablation on TS-Bench-Dojo ($1{,}220$ steps; $868$ safe and $352$ unsafe), comparing the Safety-only baseline against our Safety+RS recipe under identical data and optimization settings through the first $100$ RL iterations.

\paragraph{Safe Risk Source feedback strengthens safe-step discrimination from SFT onward.}
As illustrated in Figure~\ref{fig:agentdog-step-ablation}, incorporating Risk Source targets on safe steps already lifts Safe F1 from $94.74\%$ to $96.23\%$ at the SFT stage.
Requiring the guard to identify the origin of risk even on safe steps encourages a clearer boundary between risky contexts handled safely and genuinely unsafe actions.

\paragraph{Risk Source rewards sustain safe-group updates and consistently improve Safe F1 during RL.}
As further shown in Figure~\ref{fig:agentdog-step-ablation}, variance-filtered GDPO amplifies this difference throughout RL.
Under Safety-only feedback, safe rollout groups rapidly saturate on binary accuracy and drop out of policy updates, with safe-group participation falling to $10.9\%$ by iteration~100.
In contrast, scoring Risk Source on safe steps mitigates this reward-variance asymmetry and keeps safe-group participation at $41.8\%$ at iteration~100---roughly $3.8\times$ the Safety-only rate.
As a result, Safety+RS maintains higher Safe F1 than Safety-only at every matched RL checkpoint and further improves over its SFT baseline to reach $96.87\%$ at iteration~100, confirming that preserving safe-group learning signals strengthens safe-step discrimination.

\begin{figure*}[htbp]
  \centering
  \includegraphics[width=0.92\linewidth]{figures/step/agentdog-step-ablation.pdf}
  \caption{\textbf{Training dynamics and safe-step discrimination on TS-Bench-Dojo.}
    Panel~(a) compares the share of safe rollout groups admitted into GDPO updates under Safety-only and Safety+RS feedback during RL.
    Panel~(b) traces Safe F1 from SFT through iteration~100, with horizontal dotted lines marking each model's SFT baseline.}
  \label{fig:agentdog-step-ablation}
\end{figure*}
